Higher discrete homotopy groups of graphs

This paper studies a discrete homotopy theory for graphs introduced by Barcelo et al. We prove two main results. First we show that if $G$ is a graph containing no 3- or 4-cycles, then the $n$th discrete homotopy group $A_n(G)$ is trivial for all $n\geq 2$. Second we exhibit for each $n\geq 1$ a natural homomorphism $\psi:A_n(G)\to \mathcal{H}_n(G)$, where $\mathcal{H}_n(G)$ is the $n$th discrete cubical singular homology group, and an infinite family of graphs $G$ for which $\mathcal{H}_n(G)$ is nontrivial and $\psi$ is surjective. It follows that for each $n\geq 1$ there are graphs $G$ for which $A_n(G)$ is nontrivial.

==> sections/fakesusproof.tex <==
\begin{lemma}
If $S_t\g$ is contractible, then $t=2$ or $\g$ is contractible.

\begin{proof}
Suppose that $t>2$ and $\g$ is not contractible. Let $f:S\g\times I_m\to S\g$ be a graph map with $m\geq 1$ and $f(v_i,0)=v_i$ for all $v_i\in SG$. We claim that there is a graph map $g:G\times I_m$ such that for any $(v,i,j)\in G\times I_t\times I_m$ we have
\begin{equation}
f(v_i,j)=g(v,j)_i.
\label{eq:contra2}
\end{equation}
The lemma will follow immediately, since $f(-,m)$ cannot be a constant map. We proceed by induction on $m$. If $g(-,0):G\to G$ is the identity map, then clearly \eqref{eq:contra2} holds for $m=0$, proving the base case.

Suppose that the claim holds for $m=0,\ldots,\ell$. We show that it holds for $m=\ell+1$ as well. For $(v,i)\in G\times I_t$, we call $i$ the \emph{level} of $v_i\in S\g$. Let $g:G\times I_{\ell+1}\to G$ be a graph map such that \eqref{eq:contra2} holds for $j=0,\ldots,\ell$. It follows that the level of $f(v_i,j)$ is $i$ for all $(v,i)$ and $j=0,\ldots,\ell$.

The level of $f(v_i,\ell)$ is $i$ by our inductive hypothesis, so the level of $f(v_i,\ell+1)$ must be $i-1$, $i$ or $i+1$. Suppose toward a contradiction that the level of $f(v_i,\ell+1)$ is $i+1$ for some $v\in G$ and some $0<i<t-1$. We must have
\begin{equation}
f(v_i,\ell+1)=g(v,\ell)_{i+1},
\label{eq:fgeq}
\end{equation}
since this is the unique vertex of level $i+1$ that is adjacent or equal to $f(v_i,\ell)=g(v,\ell)_i$. If $u\simeq v$, then we must have $f(u_i,\ell+1)=g(u,\ell)_{i+1}$, since this is the unique vertex that is adjacent or equal to both $f(v_i,\ell+1)=g(v,\ell)_{i+1}$ and $f(u_i,\ell)=g(u,\ell)_i$. Hence \eqref{eq:fgeq} holds for all $v$ and our chosen value of $i$. Applying similar arguments shows that $f(v_k,\ell+1)=g(v,\ell)_{k+1}$ for all $v$ and $k=1,\ldots,i$. In particular, it follows that
\[f(v_0,\ell+1)\simeq f(v_1,\ell+1)=g(v,\ell)_2\]
for all $v$. Since $f(v_0,\ell)=v_0$, we must have $f(v_0,\ell+1)=p_1$ for some $p\in G$ adjacent or equal to all vertices in the image of $g(-,\ell)$.

Suppose that such a $p\in G$ exists. Let $h:\g\times I_{\ell+1}\to \g$ given by
\[h(v,j)=\begin{cases}g(v,j)&\mbox{if }0\leq j\leq\ell\\ p&\mbox{if }j=\ell+1.\end{cases}\]
It is routine to verify that $h$ is a contraction of $\g$ to $p$. This contradicts our assumption that $\g$ is not contractible, so the level of $f(v_i,\ell+1)$ is not $i+1$ for any $v$ and $0<i<t-1$. By symmetry, the level of $f(v_i,\ell+1)$ is not $i-1$ for any $v$ and $1<i<t$. Hence the level of $f(v_i,\ell+1)$ is $i$ for all $v$ and $i=1,\ldots,t-1$.

If $0<t<t-1$, then $f(v_i,\ell+1)=u_i$ and $f(v_{i+1},\ell+1)=w_{i+1}$ for some $u,w\in G$. Since $f$ is a graph map, we must have $u_i\simeq w_{i+1}$, implying that $u=w$. It follows that for every $v\in G$ there exists $w\in G$ such that $f(v_i,\ell+1)=w_i$ for all $i=1,\ldots,t-1$. Thus if we take $g(-,\ell+1)$ to be the map $v\mapsto w$, then \eqref{eq:contra2} holds for all $v$, $i=1,\ldots,t$ and $j=\ell+1$. To complete the inductive step, we must prove the case $i=0$; the remaining case $i=t$ will follow by symmetry. In other words, we must show that $f(v_0,\ell+1)=v_0$. If not, then since $f(v_0,\ell)=v_0$, we must have $f(v_0,\ell+1)=q_1$ for some $q\in G$. Since $f(v_0,\ell+1)\simeq f(v_1,\ell+1) = g(v,\ell+1)_1$, it follows that $q$ is adjacent or equal to all vertices in the image of $g(-,\ell+1)$. Arguing as in the previous paragraph, we obtain a contradiction. Hence $f(v_0,\ell+1)=v_0$, and we are done.
\end{proof}
\end{lemma}
